Finding the Smallest Possible Exact Aggregation of a Markov Chain

Markov chains are an important tool for modelling and evaluating systems in computer science, economics, biology and numerous other fields. Thus, approximating Markov chains is a useful tool for decreasing the computational effort needed for analysis by reducing the size of the state space. So far, most approximative algorithms focused on finding approximations, which are, again, Markov chains. We remove this restriction and present an algorithm using the Arnoldi iteration. Further, we show that if these approximations are without error, they are of minimal size. Lastly, we implement the algorithm for Markov chains via the Arnoldi iteration. If another type of aggregation, so-called Exlump aggregations, can find an exact aggregation for a Markov chain, they usually yield similar or smaller errors at much lower runtime. On the contrary, approximations computed via the Arnoldi iteration can find usable aggregations where Exlump yields none. Still, runtime is a primary concern, as our criterion for determining the approximate state space size is exceptionally costly. As such, further work is needed to decrease the runtime of the Arnoldi approach.

==> abstract.tex <==
\vspace*{2cm}
\begin{center}
    \textbf{Abstract}
\end{center}

\vspace*{1cm}

\noindent Markov chains are an important tool for modelling and evaluating systems in computer science, economics, biology and numerous other fields.
Thus, approximating Markov chains is a useful tool for decreasing the computational effort needed for analysis by reducing the size of the state space.
So far, most approximative algorithms focused on finding approximations, which are, again, Markov chains.
We remove this restriction and present an algorithm using the Arnoldi iteration.
Further, we show that if these approximations are without error, they are of minimal size.
Lastly, we implement the algorithm for Markov chains via the Arnoldi iteration.
If another type of aggregation, so-called Exlump aggregations, can find an exact aggregation for a Markov chain, they usually yield similar or smaller errors at much lower runtime.
On the contrary, approximations computed via the Arnoldi iteration can find usable aggregations where Exlump yields none.
Still, runtime is a primary concern, as our criterion for determining the approximate state space size is exceptionally costly.
As such, further work is needed to decrease the runtime of the Arnoldi approach.

\vspace*{2cm}

\begin{center}
    \textbf{Kurzfassung}
\end{center}

\vspace*{1cm}

\noindent Markov-Ketten sind ein wichtiges Instrument zur Modellierung und Bewertung von Systemen in der Informatik, den Wirtschaftswissenschaften, der Biologie und vielen anderen Disziplinen.
Das Approximieren von Markov-Ketten ist daher wichtig, um den Rechenaufwand zur Analyse zu verringern, indem die Zustandsgröße verkleinert wird.
Bislang konzentrierten sich die meisten Algorithmen auf das Finden von Approximationen, die wieder Markov-Ketten sind.
Wir heben diese Einschränkung auf und stellen einen Algorithmus vor, der die Arnoldi-Iteration verwendet, um solche Näherungen zu berechnen.
Außerdem zeigen wir, dass diese Approximationen, wenn sie keine Fehler aufweisen, von minimaler Größe sind.
Schließlich implementieren wir die Approximationsmethode für Markov-Ketten über die Arnoldi-Iteration.
Wenn eine andere Art der Aggregation, die so genannten Exlump-Aggregationen, eine exakte Aggregation für eine Markov-Kette finden kann, führt sie in der Regel zu ähnlichen oder kleineren Fehlern bei deutlich geringerer Laufzeit.
Andererseits finden Näherungen, die über die Arnoldi-Iteration berechnet werden, sogar brauchbare Aggregationen, wo Exlump keine liefert.
Dennoch ist die Laufzeit ein großes Problem, da unser Kriterium zur Bestimmung der Größe des approximierten Zustandsraums sehr zeitintensiv ist.
Daher ist weitere Arbeit erforderlich, um die Laufzeit des Arnoldi-Ansatzes zu verringern.


==> declaration-unibw.tex <==
\cleardoubleevenemptypage

\thispagestyle{empty}

\begin{large}

\vspace*{2cm}

\noindent
I hereby declare that I have written this thesis independently and without outside help, that I have properly labelled the citations and that I have not used any sources or aids other than those listed in the bibliography.\\[1em]

\noindent
Furthermore, I have taken note of the information sheet on the use of student theses and grant the University of the Bundeswehr Munich the non-exclusive right to use my bachelor's thesis.

\vspace{3cm}

\noindent
Hiermit versichere ich, die vorliegende Arbeit selbständig und ohne fremde Hilfe verfasst, die Zitate ordnungsgemäß gekennzeichnet und keine anderen, als die im Literatur/Schriftenverzeichnis angegebenen Quellen und Hilfsmittel benutzt zu haben.\\[1em]

\noindent
Ferner habe ich vom Merkblatt über die Verwendung von studentischen Abschlussarbeiten Kenntnis genommen und räume das einfache Nutzungsrecht an meiner Bachelorarbeit der Universität der Bundeswehr München ein.

\vspace{2cm}

\noindent
Munich/München, \Dday

\vspace{3cm}

\hspace*{7cm}
\dotfill\\
\hspace*{9.0cm}
\textit{(Signature/Unterschrift)}

\end{large}


==> titel-unibw.tex <==
\thispagestyle{empty}

\begin{center}

\vspace*{1cm}

\includegraphics[width=0.6\textwidth]{unibw_athene_neu}

\vspace{1.5cm}
{\Huge
\textbf{\Dtitel}\\
}
\vspace{1.5cm}


{\Large
\Dthesis \ of\\
\Dname\\
\Dnumber\\
}

\vfill

{\Large
University of the Bundeswehr Munich\\
Department of Computer Science\\
}


\end{center}

\newpage

\thispagestyle{empty}
\cleardoublepage

\thispagestyle{empty}

\begin{center}

\vspace*{1cm}

\includegraphics[width=0.6\textwidth]{unibw_athene_neu}

\vspace{1.5cm}
{\Huge
\textbf{\Dtitel}\\
}
\vspace{1.5cm}


{\Large
\Dthesis \ of\\
\Dname\\
\Dnumber\\
}
\vspace{2cm}

\parbox{1cm}{
\begin{large}
\begin{tabbing}
Supervisor: \hspace{1.5cm} \= \Dprofa \\[2mm]
Second Examiner: \> \Dprofb \\[2mm]
Advisor:
\> \Dadvisora \\
%\> \Dadvisorb \\
%\> \Dadvisorcs
\\[5mm]
Submission date: \> \Dday \\
\end{tabbing}
\end{large}}\\
\vspace{5mm}

\vfill

{\Large
University of the Bundeswehr Munich\\
Department of Computer Science\\
}

\end{center}

